Exploration of Fine-Grained Parallelism for Load Balancing Eager K-truss on GPU and CPU

In this work we present a performance exploration on Eager K-truss, a linear-algebraic formulation of the K-truss graph algorithm. We address performance issues related to load imbalance of parallel tasks in symmetric, triangular graphs by presenting a fine-grained parallel approach to executing the support computation. This approach also increases available parallelism, making it amenable to GPU execution. We demonstrate our fine-grained parallel approach using implementations in Kokkos and evaluate them on an Intel Skylake CPU and an Nvidia Tesla V100 GPU. Overall, we observe between a 1.261. 48x improvement on the CPU and a 9.97-16.92x improvement on the GPU due to our fine-grained parallel formulation.

==> Ktruss GraphChallenge 2019 cam ready plus IEEE copyright/conclusions.tex <==
This paper presents a Kokkos implementation of the Eager K-truss algorithm 
%, presented in \cite{low2018linear}, 
and improves performance by exploiting fine-grained parallelism. 
%We described the possible source of load-imbalance in graph datasets as a potential cause of reduced performance in the existing algorithm. With this as motivation, we proposed a finer-grained fine-grained parallel approach to eager K-truss. Finally, we tested and 
We presented results for our fine-grained approach of Eager K-truss on both CPU and GPU, showing that fine-grained parallelism gives significantly improved performance on GPUs and some benefits on the CPU system. By switching parallelism strategies, we observe a mean improvement of 16.93x and 9.97x on the GPU for $K=3$ and $K=K_{max}$, respectively, and an improvement on the CPU of 1.48x and 1.26x for the two $K$ settings.

%Finally, the importance of choosing the correct parallel approach on the GPU is made clear by the difference in performance between the two GPU implementations: a factor of 16.93x.

An alternative to the presented parallel approach is hierarchical parallelism (team parallelism in Kokkos) for expression of ultra-fine-grained parallelism and further improved workload balancing. In addition, while the fine-grained approach generally performs well on both platforms, larger graphs tend to show nearly the same performance on the GPU for both approaches. Determining the source of this behavior will be the subject of future work.

Graph rebalancing via full or partial sorting is another strategy to improve load-balancing \cite{Balaji:2019:CDD:3307681.3326609}. This approach could complement our fine-grained parallelism for Eager K-truss and warrants further investigation. Finally, our fine-grained approach may enable speedups in other motif-counting problems, such as butterfly counting for bipartite networks \cite{Wang2014,sanei-mehri_butterfly_2018}.


==> Ktruss GraphChallenge 2019 cam ready plus IEEE copyright/eagar.tex <==
%The eager K-truss algorithm is an edge-centric algorithm for computing the K-trusses of a graph, that was derived from a linear algebraic formulation of the K-truss operation~\cite{}. The algorithm derives its name for the eager manner in which it updates the support values of all edges for each triangle that has been identified. This is in contrast to other edge-centric algorithm that computes the support value of an edge independent of other edges that form a triangle~\cite{}. Of note, as the work by Low et al., we specifically address K-truss for undirected graphs.

% Kyungjoo
% Tze Meng is a coauthor of this paper. It sounds a bit weird that we mention his name as like someone we don't know. 
To keep this paper self-contained, we provide a brief description of the Eager K-truss algorithm in this section. For the detailed algorithmic derivation, we refer to Low et al.~\cite{low2018linear}.

\subsection{Linear Algebraic K-truss Algorithm}

Similar to many other K-truss implementations, Eager K-truss takes a two-step approach. Specifically, the first step computes the support of all edges, and the second step prunes edges whose support are below a specified threshold. This two-step approach is then repeated on the pruned graph(s) until no more edges can be removed. 
\begin{algorithm}[tb]
\small
\KwIn{$A$ is the adjacency matrix of input graph}
\KwOut{$S$ represents the support of edges in $A$}
\BlankLine                                                    
$converge \leftarrow false$\\
\While{not $converge$} {
  $S \leftarrow A^T A \circ A$ \tcp*[h]{Step 1: computeSupports}\\
  $M \leftarrow S \geq (k-2)$ \tcp*[h]{Step 2: pruneEdges}\\
  $A \leftarrow A \circ M$ \\
  $converge \leftarrow isUnchanged(M)$\\
  }
  \Return{$S$} \\
  \caption{Linear algebraic K-truss algorithm. Lowercase letters are vectors and capital letters are matrices.}
  \label{alg:linear-alg-ktruss}
\end{algorithm}

These two steps of the K-truss algorithm can generally be expressed using linear algebraic notation as described in Algorithm~\ref{alg:linear-alg-ktruss}, 
where $A$ is given as the adjacency matrix of the input graph, and $M$ is a binary matrix where $M[i,j]=1$ when $S[i,j] \geq (k-2)$ \cite{burkhardt_graphing_2017}. The $\circ$ operator represents an element-wise multiplication of the input operands.
% Kyungjoo uses algorithm package
%These two steps of the K-truss algorithm can be expressed using linear algebraic notation as follows:
%\[
%\begin{array}{rcl}
%\mbox{Step 1} \\
%S &=& A_i^TA_i \circ A_i \\
%\mbox{Step 2} \\
%M &=& S \geq (k-2) \\
%A_{i+1} & = & A_i  \circ M, 
%\end{array}
%\]
%where $A_i$ is the adjacency matrix of the input graph in the $i^{th}$ iteration of the two-step approach, and $M$ is a binary matrix where $M[i,j] =1$ when $S[i,j] \geq (k-2)$. The $\circ$ operator represents an element-wise multiplication of the left and right operand. 
Note that Step 1 computes matrix $S$, where each value at $S[i,j]$ is the number of triangles containing the edge between nodes $i$ and $j$.

\subsection{Eager K-truss Algorithm}
The Eager K-truss algorithm derives its name for the eager manner in which it updates the support values of all edges for each triangle that has been identified. Specifically, the support of all three edges that form a triangle is updated by the edge with the smallest two vertex labels.
%
%The Eager algorithm considers a graph as undirected and stores only the upper triangular part of an adjacency matrix in a compressed sparse row (CSR) format. The algorithm computes the support of edges by processing each row of the adjacency matrix in parallel. 
By re-arranging $S \leftarrow A^T A \circ A$, using a block-partitioned matrix form, the first step of the Eager K-truss algorithm is described in Algorithm~\ref{alg:eager-ktruss}. To be consistent with the notation used in \cite{low2018linear}, we use upper-case, lower-case and Greek letters to represent matrices, column vectors, and scalar elements, respectively. Since Eager K-Truss specifically focuses on undirected and unweighted graphs, it uses the upper triangular adjacency matrix in its computations. Therefore, the adjacency matrix A used in algorithm \cite{low2018linear} is upper-triangular.

Iterating over the rows of the adjacency matrix $A$ and exploiting the symmetry of the undirected graph, the computation of the support matrix $S$ follows two updating rules: lines 3 and 4 depicted in Algorithm~\ref{alg:eager-ktruss}. From now on we will refer to these as the $s_{12}$ and $S_{22}$ update rules, respectively. As data dependencies exist among different iterations, the updates are performed in an atomic fashion.

In essence, the Eager algorithm in Algorithm \ref{alg:eager-ktruss} computes edge supports by performing set intersections for vertex neighborhoods on either side of a current edge and updating all edges in each triangle found. Neighborhood intersections are grouped by their common source vertex, whose outgoing neighborhood is $a_{12}$. Imbalances can occur since vertices do not have identically sized outgoing neighborhoods.
%Also, note that $\alpha_{11}$ is equal to zero because it is on the main diagonal of a symmetric graph with no self loops. 
%A single iteration $i$ of K-truss is then executed by the Eager algorithm by computing the update rules for each overall partitioning of $A$, such that each partitioning has an $a_{i_{12}}^T$ vector and an $A_{i_{22}}$ matrix defined in the lower right quadrant of that partitioning. With eager K-truss described to this level of detail, we now describe issues of load balancing in the following section.

\begin{algorithm}[tb]
  \footnotesize
  \KwIn{$A$ is the upper-triangular adjacency matrix of the input graph}
  \KwOut{$S$ represents the support of edges in $A$}
  \BlankLine
  \SetKwFor{ParFor}{parallel for}{do}{end}
  \ParFor{ $i\ in\ range(0,numRows(A))$ } {
    partition $A$ and $S$ where $\alpha_{11}$ and $\sigma_{11}$ are scalar corresponding to the diagonal values of $A_{ii}$ and $S_{ii}$ as follows:
    {\scriptsize $\left(\begin{array}{c|cc}
    A_{00} & a_{01} & A_{02} \\ \hline
    \quad  & \alpha_{11} & a_{12}^T \\
    \quad  & \quad       & A_{22} \\
    \end{array}\right)
    $ } and
    {\scriptsize $\left(\begin{array}{c|cc}
    S_{00} & s_{01} & S_{02} \\ \hline
    \quad  & \sigma_{11} & s_{12}^T \\
    \quad  & \quad       & S_{22} \\
    \end{array}\right)
    $ }
    \\
    $s_{12}^T \leftarrow s_{12}^T + a_{12}^T A_{22} \circ a_{12}^T$\\ 
    $S_{22}^T \leftarrow S_{22}^T + a_{12} a_{12}^T \circ A_{22}$\\
  }
  \Return{$S$}\\
  \caption{computeSupports in Eager K-truss. Greek, lower-case and upper-case letters are scalars, vectors and matrices respectively. Loop range is defined with a start value and a non-inclusive upper bound.}
  \label{alg:eager-ktruss}
\end{algorithm}
% Kyungjoo: I put this earlier
%To keep this paper self-contained, we provide a brief description of the eager k-truss algorithm and refer the interested reader to Low et. al.~\cite{low2018linear} for the details of the algorithm.
% Kyungjoo: the notation seems to be difficult to decipher.
% The union of partitioned graph G1 and G2 is not G if we refer them to ATL and ABR.
%Consider a graph $\mathcal G$ that has been partitioned into two subgraphs $\mathcal G_1$ and $\mathcal G_2$. Note that in this formulation, the graph is undirected and therefore the full adjacency matrix representing the graph $\mathcal{G}$ is symmetric. The partitions $\mathcal{G}_1$ and $\mathcal{G}_2$ can then be designated by a partitioning on the original adjacency matrix $A$ shown below:
%\[
%A=
%\left[
%\begin{array}{c|c}
%A_{TL} & A_{TR} \\
%\hline
%A_{BL} & A_{BR}
%\end{array}
%\right]
%\]
%
%Such that the graph partitions $\mathcal{G}_1$ and $\mathcal{G}_2$ are represented by the top left ($A_{TL}$) and bottom right ($A_{BR}$) of the partitioned matrix. With this partitioning in place, Low et al. then show that computing  $A_i^TA_i \circ A_i$ can be re-written in terms of the matrix quadrants \cite{low2018linear}.
%By re-arranging the decomposed expressions for enumerating the triangles in the matrix and taking advantage of the matrix symmetry, computation of the support matrix $S_i$ for a given iteration can be re-written in terms of update rules defined for matrix $S_i$ and a specific partitioning of matrix $A_i$:
%$$s_{i+1_{12}} = s_{i_{12}} + a^T_{i_{12}} A_{i_{22}} \circ a^T_{i_{12}}$$
%$$S_{i+1_{22}} = S_{i_{22}} + a_{i_{12}}a^T_{i_{12}} \circ A_{i_{22}}$$
%
%From now on we will refer to these as the $s_{12}$ and $S_{22}$ update rules, respectively. The input vector $a_{i_{12}}$ and input matrix $A_{i_{22}}$ are defined by the partitioning the sub-matrix $A_{BL}$ once more, such that:
%\[
%A_{BR}=
%\left[
%\begin{array}{c|c}
%\alpha_{i_{11}} & a^T_{i_{12}} \\
%\hline
%a_{i_{12}} & A_{i_{22}}
%\end{array}
%\right]
%\]
%Where $\alpha_{i_{11}}$ is equal to zero because it is on the main diagonal of a symmetric graph with no self loops. A single iteration $i$ of k-truss is then executed by the eager algorithm by computing the update rules for each overall partitioning of $A$, such that each partitioning has an $a_{i_{12}}$ vector and an $A_{i_{22}}$ matrix defined in the lower right quadrant of that partitioning. With eager K-truss described to this level of detail, we now describe issues of load balancing in the following section.

==> Ktruss GraphChallenge 2019 cam ready plus IEEE copyright/implementation.tex <==
% \subsection{Approaches to Fine-Grained Parallelism}

% No longer relevant:
% Kokkos supports expression of hierarchical parallelism in which 
% teams of threads operate in parallel on sections of work. This 
% layered parallelism extend to three levels, including a vector-level
% parallelism that roughly corresponds to SIMD on CPUs and warps or 
% thread groups on GPUs. The fine-grained parallel approach can be augmented 
% with team parallelism, either by parallelizing over elements of A22,
% elements of a12, or both. We refer to the first two as \textit{vector}-
% parallel and the latter as \textit{outer-product} parallel.

% Single-level parallelism (range parallelism) can be augmented by chunking work items; 
% that is, parallel workers will be assigned a set of $n$ work items 
% in a round robin fashion, rather than 1 work item. 
% Chunking parallel items is analogous in work distribution to 
% block-cyclic data distribution, as a task of a single work item is to
% element-cyclic data distribution.
% % Could also be compared to loop unrolling.
% Creating chunks of work items can reduce the overhead of parallelism,
% while still keeping imbalance low as long as individual work items are 
% similarly sized. In our results we refer to this approach as 
% \textit{chunk}-parallel.

\begin{minipage}{0.97\linewidth}
\begin{lstlisting}[language=C++, caption=Fine-grained support computation in  Kokkos,label=lst:fine-grained-eager-kokkos]
using namespace Kokkos;
using SpT = Cuda; // Serial, OpenMP, Cuda
using IJ_ViewType = View<uint32_t*,SpT>;
// ++, += operators are overloaded by atomic updates
using S_ViewType = View<uint16_t,SpT,MemoryTraits<Atomic> >;
// CSR input (IA and JA) and support matrix S are stored on device memory
uint32_t fine_grained_parallel_eager(
  IJ_ViewType IA, IJ_ViewType JA, // CSR input of a graph (matrix A) 
  S_ViewType S, // support of edges
  uint32_t K) // K-truss parameter
  const uint32_t nnz = JA.extent(0), nverts = IA.extent(0)-1;
  uint32_t tri_new(1);
  while (tri_new) {
    tri_new = 0;
    // Step 1: computeSupports
    parallel_for(RangePolicy<SpT>(0, nnz),
      KOKKOS_LAMBDA(const uint32_t ij) const {
        auto a12_pred = JA(i);
        if (a12_pred != 0) {
          auto a12_start_off = i+1;
          auto A22_start_off = IA(a12_pred);
          auto A22_end_off = IA(a12_pred+1)-1;
          uint16_t SL(0);
          while (JA(a12_start_off)!=0 && JA(A22_start_off)!=0){
            const auto flag = (JA(A22_start_off) == JA(a12_start_off));
            if (flag) {
              ++(S(a12_start_off));
              ++(S(A22_start_off));
              SL++;
              a12_start_off++;
              A22_start_off++;
            } else if (JA(A22_start_off) > JA(a12_start_off)){
              a12_start_off++;
            } else {
              A22_start_off++;
            }
          }
          S(i) += SL;
        }
      });
    fence();
    pruneEdges();   // Step 2 (omitted due to space constraints)
  }
  return tri_new;
}
\end{lstlisting}
\vspace{-3mm}
\end{minipage}

    % // Step 2: pruneEdges
    % parallel_reduce(RangePolicy<SpT>(0, nverts), 
    %   KOKKOS_LAMBDA(const uint32_t i, uint32_t &update) const {
    %     const auto start = IA(i);
    %     auto nnz_j(start);
    %     auto j(start);
    %     while (JA(j)!=0) {
    %       const swp = JA(j);
    %       JA(j) = 0;
    %       if (S(j) >= K-2) {
    %         JA(nnz_j) = swp;
    %         nnz_j++;
    %       }
    %       S(j) = 0;
    %       j++;
    %     }
    %     if (nnz_j < j) update += 1;
    %   }, tri_new);

\subsection{Performance Portable Implementation via Kokkos}

Kokkos provides a performance portable parallel programming model with node-level device abstractions i.e., execution space, memory space, execution policy and parallel patterns. %As we cannot explore all opportunities provided by Kokkos, 
We briefly explain Kokkos features that we primarily used for our fine-grained-parallel implementation. An execution space and a memory space define where the code is executed and where data resides. For example, an execution space supports Serial, OpenMP and Cuda for GPUs while a memory space includes HostSpace, CudaUVMSpace (host accessible) and CudaSpace. Then, a device can be described as a combination of an execution space and corresponding memory space. An execution policy defines how computing units are mapped to concurrent tasks. In our implementation, we use  RangePolicy that maps a single thread to a single work unit defined in a range of an iteration space. Kokkos also provides commonly used parallel algorithms i.e., parallel for, reduce, and scan, which are interfaced via a functor provided by users. 

Listing~\ref{lst:fine-grained-eager-kokkos} illustrates the implementation of fine-grained support computation using Kokkos. The pruning subroutine is identical to \cite{low2018linear} and is omitted for brevity. As input, the code expects an upper-trianglular CSR input matrix of $IA$ and $JA$ arrays where they represent row pointers and column indices. $S$ indicates an array for storing edge supports and the array is decorated with an Atomic memory trait. Using Kokkos, this code works for both CPUs and NVIDIA GPUs by changing a single line of the code specifying an execution space. Note that while we use a flat range policy in the implementation, Algorithm~\ref{alg:fine-ktruss} is expressed as nested parallel for readability. %A detailed flattening strategy of $(i,j)$ pair indices is described in the next. 

\subsection{Zero-terminated CSR}
%% Mark : I kind of change some notations. Would you change accordingly ? -Sure!
Recognize that  %In implementing our fine-grained parallel approach, we realized that 
the information determining which $a_{i,j_{12}}$ and $A_{i,j_{22}}$ (notated $A(\kappa, :)$ in Algorithm~\ref{alg:fine-ktruss}) sub-vectors are used as inputs to a particular task is almost entirely characterized by the location and contents of the element in $a_{i,j_{12}}$ located at $A(i,j)$. By defining each task based on the matrix element, we are able to avoid adding an additional data structure for tracking tasks. %This is significant as the number of tasks is proportional to the number of edges which is typically much larger than the number of vertices.
%In order to avoid the aforementioned additional data structure, 

However, we did modify the triangularized CSR graph representation such that 
%instead of storing each vertex neighborhood contiguously in an array of length equal to number of edges, we terminate 
each vertex neighborhood is terminated with an additional zero value. This increases the length of the entire vector of non-zero elements by the number of vertices, but allows the ends of each task's input vectors to be implicitly coded without external bookkeeping. %, which is often much smaller than the number of edges, $E$. %With regards to algorithmic implementation, 
This change is minor because the pruning step already introduces zeros as a way of implementing early termination. Therefore, zero-terminating the rows at the start simplifies the implementation and enables fine-grained parallel implementation.
%from the start does not change logic already designed to deal with the matrix as it becomes sparser. 
%Hence, this change is compatible with the existing pruning approach while enabling fine-grained parallel operation.



==> Ktruss GraphChallenge 2019 cam ready plus IEEE copyright/intro.tex <==
%Graph analytics and graph processing workloads have exploded in relevance to today's
%industrial, commercial, research, and national security applications. 
%In tandem, the scale of data has grown ferociously, consuming all of the computational power 
%that modern high-performance computing (HPC) systems have to offer.
%The third trend shaping high performance graph processing is that of diverse architectures, which 
%each have their own benefits for HPC, but across which obtaining portable performance
%is a laborious endeavor.
%This difficulty stems in part from incomplete understanding of the graph algorithms 
%themselves, as well as how to best apply these algorithms to the varying graph types, 
%diverse hardware, and programming models available today.

%{\bf I would remove these two para}
%The GraphChallenge is an organized effort to forward the high-performance graph community's
%understanding of graph algorithms and the performance issues faced at the scale of today's 
%data and systems. Every year the GraphChallenge invites researchers to work on a set of 
%graph problems highlighted as important to building the community's understanding. 
%
% One of the graph problems presented starting in 2017 is K-truss\cite{graphchallenge:Isomorphism:2017}. 

% {\bf sounds like a repeat}
% K-truss is characterized by iterating on a two-step process. 
% The first step is triangle enumeration, in which the number of triangles, or 3-cliques, in the
% graph are enumerated and the number of triangles in which an edge participates recorded.
% This value is typically termed `support' of an edge.
% The second step is a pruning stage, in which each edge that has a support value strictly
% less than `K-2', derived from the user-input term K, is removed.
% Removal of edges from the graph may well break triangles that were previously found, thus
% necessitating iteration of the two phases until a steady state is reached.
% If a stable sub-graph remains, this graph is known as the `K-truss' of the graph and can
% be used in further studies as a highly connected and clustered subgraph of the original.

The K-trusses of a graph $\mathcal G$ are highly connected subgraphs of $\mathcal G$
where each edge in a subgraph is an edge in at least $K-2$ distinct triangles in the 
subgraph~\cite{cohen2008trusses}. 


%% Kyungjoo
%% 
In this work, we present a fine-grained parallel implementation of the Eager K-truss algorithm\cite{low2018linear}, a linear algebraic formulation of an edge-centric K-truss algorithm, on both the CPU and the GPU. The key observation is that the
existing Eager K-truss algorithm uses a coarse-grained approach to parallelism by dividing the edges into blocks that are distributed between parallel workers based on the common vertex that the edges are connected to; typically the `source' vertex. As each edge may be connected to different number of neighboring edges (i.e. edges that share the same vertex), the performance of this approach suffers from potential load imbalance. In addition, the Eager K-truss algorithm computes with an upper-triangular adjacency matrix, which means this load imbalance may be skewed significantly as the algorithm proceeds. 

We resolve the load imbalance problem by introducing a finer-grained task unit upon which parallel workers compute edge membership in triangles - the edge support values. This, in essence, introduces parallelism within each block of edges assigned to a processing element.
%, which significantly improves the number of concurrent tasks. 

In Sections~\ref{sec:eager} and \ref{sec:fine-grained-eager}, we present details of our proposed algorithm. For an efficient implementation, we use a performance portable parallel programming model, Kokkos\cite{Edwards:2014:kokkos}. In particular, we report our K-truss performance for several fixed K values on NVIDIA V100 and Intel Skylake architectures. We report our results in millions of edges processed per second for each graph, and provide a summary table with timings in milliseconds for specific configurations.

% Mark version
%In a previous submission to the GraphChallenge, on of our authors presented a linear-algebraic approach to an edge-centric k-truss algorithm \cite{low2018linear}. However, while our previous approach parallelized on the CPU cores of a shared-memory system, it was noted that certain graphs caused imbalance in the work allocated to each thread worker. In addition, our initial implementation was based on OpenMP and could not be used to explore performance on GPUs \cite{}. In this work, we present a finer-grained parallelism approach to improve load balancing and amount of parallel work on GPUs, in contrast to our original CPU-only version. 

==> Ktruss GraphChallenge 2019 cam ready plus IEEE copyright/kokkos.tex <==
Performance portability, particularly for parallel algorithms,
is a major challenge for developers in HPC.
In this study, we seek to test our parallel-algorithmic approach to 
load balancing on both CPU and GPU platforms.
To code portability, we used the Kokkos parallelism framework to express 
flattened and nested parallel loops for kernels in eager K-truss. \cite{}
The Kokkos framework and runtime ?? enable such parallel applications to be written 
once and recompiled for shared-memory HPC platforms that used CPUs and GPUs.
Management of memory, including arbitration of atomic accesses and data layout 
are also handled by the Kokkos framework.

While in our testing we found that some performance was lost between our original
OpenMP C implementation of eager K-truss and the direct C++ port in Kokkos, 
the benefit was being able to test and deploy our implementations across both 
CPU and GPU hardware with minimal changes to code. 
Other frameworks for portable parallelism and performance include OpenCL, OpenACC,
and OpenMP itself \cite{}. 
We acknowledge these frameworks; however our objectives in this work do not include
a performance comparison between these different frameworks.


==> Ktruss GraphChallenge 2019 cam ready plus IEEE copyright/load_balancing.tex <==
% Kyungjoo
\subsection{Source of Load Imbalance in Eager K-truss}
%\subsection{Load Balancing Parallelism in Eager K-Truss}

%Kyungjoo
% can we use i for partitioning instead of j ?
% iteration count is not really meaningful in 
% describing the algorithm

For each matrix partitioning $i$ at a given iteration, the $s_{12}$ and $S_{22}$ update rules are applied. %One can easily notice that the
As matrix $A$ is upper triangular,  the computational cost of the two updates may decrease as the iteration count $i$ increases. %Although this may not be precisely true and the actual number of updates is dependent on the sparsity pattern and ordering of an input graph, we can in practice assume this because the $S_{22}$ update performs an outer product on an upper triangular block. 
Further, the imbalanced nature of the graph connectivity can lead to significant performance degradation especially when a large number of computing units are used in parallel. Intuitively, this imbalance arises in part from the decrease in length of vector $a_{i_{12}}^T$ and also from the shrinking size, both in width and height, of the sub-matrix $A_{i_{22}}$. However, because the matrix $A$ is typically highly sparse, the width and height of $A_{i_{22}}$ is far less relevant than the number of non-zero elements in $a_{i_{12}}^T$. Even the number of non-zero elements in $A_{i_{22}}$ does not directly influence imbalance. The major reason for this is that the number of row vectors in $A_{i_{22}}$ that are relevant to the update rules is directly determined by the non-zero elements present in $a_{i_{12}}^T$. 

%To test this intuition, we measured the number of edge updates performed by the two update rules for each partition iteration $i$ for various graphs from the Stanford Network Analysis Project (SNAP)~\cite{snap:2014}. We found that for both road networks with low and uniform degree distribution and scale free networks with power law distribution, the number of non-zero elements in $A_{i_{22}}$ was indeed irrelevant; if an edge from the vertex represented by the current $a_{i_{12}}^T$ to a particular row of $A_{i_{22}}$ did not exist then none of the elements in that part of $A_{i_{22}}$ would be accessed. Instead we noticed that the number of actual updates tends to be related to the number of non-zero elements in $a_{i_{12}}^T$. Therefore, we suggest a straightforward strategy for load balancing the Eager K-truss algorithm based on the non-zero elements in $a_{i_{12}}^T$.

\subsection{Fine-grained Tasks for Updating Edge Supports}

\begin{algorithm}[tb]
  \footnotesize
  \KwIn{$A$ is the upper-triangular adjacency matrix of the input graph}
  \KwOut{$S$ represents the support of edges in $A$}
  \BlankLine
  \SetKwFor{ParFor}{parallel for}{do}{end}
  \ParFor{ $i\ in\ range(0,numRows(A))$ } {
    partition $A$ and $S$ where $\alpha_{11}$ and $\sigma_{11}$ are scalar corresponding to the diagonal values of $A_{ii}$ and $S_{ii}$ as follows:
    {\scriptsize $\left(\begin{array}{c|cc}
    A_{00} & a_{01} & A_{02} \\ \hline
    \quad  & \alpha_{11} & a_{12}^T \\
    \quad  & \quad       & A_{22} \\
    \end{array}\right)
    $ } and
    {\scriptsize $\left(\begin{array}{c|cc}
    S_{00} & s_{01} & S_{02} \\ \hline
    \quad  & \sigma_{11} & s_{12}^T \\
    \quad  & \quad       & S_{22} \\
    \end{array}\right)
    $ }
    \\
    \ParFor{$j\ in\ nonZeros(a_{12}^T)$} {
      $\kappa \leftarrow a_{12}^T(j)$ \tcp*[h]{index of $A_{22}$ row w.r.t $A$} \\      
      \tcp{$A(\kappa,:)$ is the row in $A_{22}$ for task $(i,j)$} 
      \tcp{$S(\kappa,:)$ is the row in $S_{22}$ for task $(i,j)$}
      $s^T_{12}(j) \leftarrow s^T_{12}(j) + A_{22}(\kappa, :)a_{12}$ \\
      $s_{12}^T(j+1:) \leftarrow s_{12}^T(j+1:) + a_{12}^T(j+1:) \circ A(\kappa,:)$\\
      $S(\kappa,:) \leftarrow S(\kappa,:) + a_{12}^T(j+1:) \circ A(\kappa,:)$\\
    }
  }
  \Return{$S$}
  \caption{computeSupports in fine-grained Eager K-truss. 
  Greek, lower-case and upper-case letters are scalars, vectors and matrices respectively.
  %Greek lowercase letters are scalars, lowercase letters are vectors, and capital letters are matrices. 
  Loop and vector or matrix dimension ranges are defined with a start value, colon, and either a non-inclusive upper bound or no upper limit indicating inclusion of the remaining space.}
  \label{alg:fine-ktruss}
\end{algorithm}

\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{plots/task_work_breakdown.pdf}
    \caption{Partitioning $i$ corresponding to a specific set of inputs to the support updates. The left side illustrates that the 
    %; while $A_{i_{22}}$ and $a_{i_{12}}^T$ are indeed sparse, 
    the work is roughly proportional to the number of non-zero elements in $a_{i_{12}}^T$. The right side shows a fine-grained set of tasks, where each task is further refined by the $i^{th}$ partitioning and the $j^{th}$ non-zero value in $a_{i_{12}}^T$. Task $(i,j)$ updates $s_{12}$  on the $i^{th}$ row, and a row in $S_{22}$ indicated by the $j^{th}$ value in $a_{i_{12}}^T$.}
    \label{fig:diff_tasks}
    \vspace{-4mm}
\end{figure}

Our load balancing strategy is to take advantage solely of the information provided by a particular $a_{i_{12}}^T$: the number of non-zero elements which directly indicate the number of neighborhoods in $A_{i_{22}}$ that must be visited. Thus, a fine-grained task can be defined as a row-wise update by selecting a row in $A_{i_{22}}$ based on the $j^{th}$ value of $a_{i_{12}}^T$, rather than updating multiple rows in $A_{i_{22}}$ from the outer product of $a_{i_{12}}^T$. As a result, our fine-grained Eager algorithm iterates over a pair iterator $(i,j)$ that corresponds to the number of non-zero elements of $A$. Fig.~\ref{fig:diff_tasks} illustrates the difference between the two parallel approaches. To distinguish these two algorithms, we refer the original Eager K-truss algorithm as \textit{coarse-grained} parallel since each parallel task in the algorithm operates on a group of edges that share the same source vertex. In contrast, we refer to our parallel approach using tasks defined by each non-zero element of the matrix as \textit{fine-grained} parallel; it is described in Algorithm~\ref{alg:fine-ktruss}.

The actual work to be performed 
is determined by both the number of non-zero elements in $a_{i_{12}}^T$ \textit{and} 
the non-zero elements within the relevant row of $A_{i_{22}}$ indicated by a non-zero value in $a_{i_{12}}^T$. Therefore, the update rules could then further divided into smaller tasks by grouping the elements within a row of $A_{i_{22}}$. However the information as to exactly how many elements of a row of $A_{i_{22}}$ should be grouped is not straightforward and precise determination of this information can cost similarly to the actual cost of applying the update rules. Therefore we leave it to future work to explore the merits of such ultra-fine-grained tasks. Finally, we note that in either approach outlined above, the Eager K-truss algorithm is still edge-centric; it is simply that the expression of parallelism is changed from parallel over groups of edges within a row (on the order of number of vertices) to parallel over tasks identified by individual edges (on the order of non-zero elements).

%
% Mark version
%For each matrix partitioning $j$ within an overall iteration $i$ of eager k-truss, the $s_{12}$ and $S_{22}$ update rules are applied for the $a_{12}$ and $S_{22}$ inputs specified by partition $j$. One may note that the number of unique partitions for the graph $\mathcal{G}$ having $N$ vertices and $V$ edges is $N$: each partition corresponds to a specific tuple ($a_{12}$, $A_{22}$). By iterating over each row in the matrix, a developer can implement a loop body that applies each of the two update rules for the partitioning specified by the loops iteration value $j$. A second important observation is that since the matrix is symmetric, values of $a_{12}$ and $A_{22}$ begin after the main diagonal. Hence, the width of each is constrained by the effectively triangular shape of the matrix $A$.
%
%Finally, such a loop can be executed in parallel
%provided appropriate locking mechanisms are used to execute $s_{12}$ and $S_{22}$ update rules 
%for all partitions in parallel.
%
%This imbalanced nature of the graph connectivity leads to a performance limitation when the approach described in Algorithm~\ref{alg:eager-ktruss} is executed in parallel. Intuitively, this imbalance may come in part from the decrease in length of vector $a_{12}$ and even more so from the shrinking size, both in width and height, of the sub-matrix $A_{22}$. In fact, because the matrix $A$ is typically highly sparse, the size of $A_{22}$ is far less relevant. One major reason for this is that the number of row vectors in $A_{22}$ that are relevant to the update rules is directly determined by the non-zero elements present in $a_12$. 

% TODO: NEED A FIGURE HERE TO ILLUSTRATE; DESCRIBE THE INNER AND OUTER PRODUCTS IN THE RULES?

%To test this intuition, we measured the number of arithmetic operations for each partition iteration $j$, due to each update rule. This was done by instrumenting the original code provided by Low et al. It was found that for both road networks with low and uniform degree distribution and scale free networks with power law distribution, the number of non-zero elements in $A_{i,j_{22}}$ was irrelevant: if an edge from the vertex represented by the current $a_{i,j_{12}}$ to a particular row/column of $A_{i,j_{22}}$ did not exist, then none of the non-zero elements in that part of $A_{i,j_{22}}$ would be accessed, no matter how many there might be. Further, for a given partition $j$, the number of non-zero elements in $A_{i,j_{22}}$ was the full number of non-zeros below row $j$, which rarely coincided with the number of actual updates performed for that partition.

%Therefore, we suggest a straightforward strategy for load balancing the eager k-truss algorithm. The strategy is to take advantage solely of the information provided by a particular $a_{i,j_{12}}$: the number of non-zero elements, which directly indicate the number of neighborhoods in $A_{i,j_{22}}$ that must be visited. By iterating over $k$ tasks based on each of $k$ elements in $a_{i_{12}}$, eager K-truss switches from iterating over each row $j$ in the matrix to iterating over tasks defined by each entry ($j,k$) in the matrix. Fig. \ref{fig:diff_tasks} illustrates the difference between the two approaches.

%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{plots/task_work_breakdown.pdf}
%    \caption{This figure shows the same matrix partitioning $j$ at iteration $i$ corresponding to a specific set of inputs to the support updates. The left side illustrates the work breakdown that occurs for iteration over rows: while $A_{i,j_{22}}$ and $a_{i,j_{12}}$ are indeed sparse, the work is roughly proportional to the number of elements ($k$) in $a_{i,j_{12}}$. The right side shows a finer-grained set of tasks, where each task is further defined by the $j$ partitioning and the $k^{th}$ non zero value in $a_{i,j_{12}}$.}
%    \label{fig:diff_tasks}
%\end{figure}

%Using non-zero matrix elements (edges) over which to process in parallel, we propose to divide work in K-truss in a fine-grained manner. By distributing $k$ rows in the sparse $A_{i,j_{22}}$ sub-matrix for a given $a_{i,j_{12}}$, more consistently sized tasks for a greater number of parallel workers can be created, thereby reducing the number of straggler processes caused by imbalanced parallelism.

%The original implementation of Low et al. operated on parallel for each row of the adjacency matrix, in a manner that we will refer to as \textit{vertex}-parallel since each row of the  matrix represents the out-going edges of a vertex. In contrast, our approach to fine-grained parallelism operates on tasks defined by each non-zero element of the matrix, which correspond to edges in the graph. From here, we refer to parallelizing over all edges as \textit{task}-parallel.

% \begin{minipage}{\textwidth}
% \begin{minipage}{0.46\textwidth}
% \begin{algorithm}[H]
% % \caption{Vertex-Parallel K-Truss}\label{Algorithm 1}
% \begin{algorithmic}[1]
% \State matrix $A_i$ at iteration $i$
% \State in parallel:
% \For {row $j$ in matrix $A_i$}
% \State select vector $a_{i,j_{12}}$
% 	\For {elem $k$ in vector $a_{i,j_{12}}$ }
% 		\State select vector $A_{i,j,k_{22}}$
% 		\State Intersect($a_{i,j,k_{12}}$, $A_{i,j,k_{22}}$)
% 	\EndFor
% \EndFor
% \end{algorithmic}
% \end{algorithm}
% % \end{minipage}
% % \hfill
% % \begin{minipage}{0.46\textwidth}
% \begin{algorithm}[H]
% % \caption{Task-Parallel K-Truss}\label{Algorithm 2}
% \begin{algorithmic}[1]
% \State matrix $A_i$ at iteration $i$
% \State in parallel:
% \For {elem $(j,k)$ in matrix $A_i$}
% 	\State select sub-vector $a_{i,j,k_{12}}$
% 	\If{elem $a_{i,j,k_{12}}$ != 0}
% 		\State select vector $A_{i,j,k_{22}}$
% 		\State Intersect($a_{i,j,k_{12}}$, $A_{i,j,k_{22}}$)
% 	\EndIf
% \EndFor
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% \end{minipage}

%It should be acknowledged that the actual work is determined by both the number of non-zero elements in $a_{i,j_{12}}$ \textit{and} the non-zeros in the $k$ relevant rows of $A_{i,j_{22}}$. The update rules could be be divided into still smaller tasks. However, the information as to exactly how many entries there will be in just the relevant rows of $A_{ij,_{22}}$ make this less straightforward than the scheme we describe above, and we leave it for future work to explore the merits of this approach. Finally, note that in either approach outlined above, eager K-truss algorithm is still edge-centric; it is simply that the expression of parallelism is changed from parallel over rows (on the order of number of vertices) to parallel over elements (on the order of number of non-zero elements).



% Not relevant to the current paper:
% The second method requires additional pre-processing, but may provide better load balancing 
% information when the sizes of neighborhoods in $A_{i_{22}}$ vary significantly.

% \subsection{Metric of Graph Imbalance}
% We propose that the amount of imbalance in a graph can be quantified by the variance in number
% of non-zero elements (NNZ) updated within the output matrix due to each of the two rules.
% For an `inner' iteration $i$, this corresponds to NNZ updates in $s_{i_{12}}$ and $S_{i_{22}}$.
% TODO: I think that using NNZ in a12 and in A22 are both proxies for the above, and if we wanted
% to evaluate both methods against each other and other strategies then we would need a 'neutral'
% metric (as above) not based directly on the method used by either method. 
% We experimentally measure this for a given graph by counting the number of updates to memory 
% locations corresponding to S22 and s12 and computing the variance across `inner' iterations.
% Todo: I am still not satisfied with this. I would like to discuss this more.

% What I really want is a metric that quantifies (potential??) load imbalance in the eager algorithm.
% Once concern I have is that if the algorithm is changed specifically to reduce load imbalance,
% then this metric would actually only be useful to correlate with the improvement we expect to see from 
% eager k-truss as-is to a unit-task parallel algorithm. It would not be directly applicable to the new
% algo, since the new one would be specifically designed to reduce load imbalance...

% One important point I want to make is that load imbalance can change with different organization 
% of the adjacency matrix, and that is fine. The work we do here should function complementarily 
% with something like sorting the graph by degree, and the metric should indeed reflect reduced 
% load imbalance in a sorted graph if it indeed runs better in eager-ktruss when sorted, 
% \textbf{assuming} that the initial performance is indeed limited by load imbalance.

% Possible experiment to validate the utility of the metric: we already know that sorting the 
% graph can give better runtime. My hypothesis is that sorting the graph decreases load 
% imbalance, which therefore improves the runtime. If I either assume that the improved runtime
% is due to reduced imbalance or actually prove it somehow, then I can use those cases to validate 
% the metric: if the runtime increases due to sorting, I should see the metric rise as well; 
% if the runtime improves, I should see the metric fall.



==> Ktruss GraphChallenge 2019 cam ready plus IEEE copyright/plots/table.tex <==
\begin{table*}[]
\scriptsize
\centering
\caption{Runtimes and ME/s Performance Numbers for all graphs tested. Postfix in subgroup heading refers to coarse or fine-grained parallelism. All CPU results presented in this table are for 48 threads, and all runs are for $K=3$.}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|cc|cccc|cccc|}
\hline
 & & &  \multicolumn{4}{c|}{Time (ms)} & \multicolumn{4}{c|}{Millions of Edges per Second (ME/s)} \\
 Input Graph           & Vertices (k) & Edges    & CPU-C     & CPU-F   & GPU-C    & GPU-F  & CPU-C                        & CPU-F   & GPU-C    & GPU-F    \\ \hline
ca-GrQc               & 5.2k         & 14.5k    & 1.660     & 1.051   & 3.982    & 0.762  & 8.724                        & 13.784  & 3.637    & 19.003   \\
p2p-Gnutella08        & 6.3k         & 20.8k    & 0.343     & 0.230   & 3.334    & 0.472  & 60.663                       & 90.178  & 6.232    & 44.028   \\
as20000102            & 6.5k         & 12.6k    & 3.715     & 1.062   & 148.729  & 1.837  & 3.384                        & 11.839  & 0.085    & 6.843    \\
p2p-Gnutella09        & 8.1k         & 26.0k    & 0.404     & 0.316   & 2.000    & 0.506  & 64.309                       & 82.242  & 13.006   & 51.409   \\
p2p-Gnutella06        & 8.7k         & 31.5k    & 0.333     & 0.303   & 1.153    & 0.320  & 94.727                       & 104.112 & 27.342   & 98.516   \\
p2p-Gnutella05        & 8.8k         & 31.8k    & 0.380     & 0.409   & 1.326    & 0.417  & 83.831                       & 77.808  & 24.015   & 76.316   \\
ca-HepTh              & 9.9k         & 26.0k    & 0.924     & 0.860   & 2.135    & 0.458  & 28.115                       & 30.191  & 12.164   & 56.660   \\
oregon1\_010331       & 10.7k        & 22.0k    & 2.511     & 1.338   & 61.248   & 1.475  & 8.763                        & 16.448  & 0.359    & 14.918   \\
oregon1\_010407       & 10.7k        & 22.0k    & 2.433     & 1.916   & 62.416   & 1.408  & 9.040                        & 11.484  & 0.352    & 15.628   \\
oregon1\_010414       & 10.8k        & 22.5k    & 2.161     & 2.023   & 63.569   & 1.428  & 10.396                       & 11.106  & 0.353    & 15.730   \\
oregon1\_010421       & 10.9k        & 22.7k    & 2.081     & 1.892   & 64.603   & 1.421  & 10.932                       & 12.021  & 0.352    & 16.011   \\
p2p-Gnutella04        & 10.9k        & 40.0k    & 0.413     & 0.319   & 0.740    & 0.241  & 96.838                       & 125.216 & 54.024   & 166.088  \\
oregon1\_010428       & 10.9k        & 22.5k    & 1.964     & 1.330   & 66.396   & 1.482  & 11.453                       & 16.916  & 0.339    & 15.174   \\
oregon2\_010331       & 10.9k        & 31.2k    & 2.938     & 2.049   & 65.880   & 1.568  & 10.613                       & 15.216  & 0.473    & 19.881   \\
oregon1\_010505       & 10.9k        & 22.6k    & 1.801     & 1.842   & 66.031   & 1.399  & 12.552                       & 12.272  & 0.342    & 16.163   \\
oregon2\_010407       & 11.0k        & 30.9k    & 2.515     & 1.860   & 64.638   & 1.846  & 12.269                       & 16.588  & 0.477    & 16.715   \\
oregon1\_010512       & 11.0k        & 22.7k    & 1.961     & 1.518   & 66.446   & 1.443  & 11.562                       & 14.937  & 0.341    & 15.713   \\
oregon2\_010414       & 11.0k        & 31.8k    & 3.120     & 2.020   & 67.370   & 1.816  & 10.180                       & 15.727  & 0.471    & 17.488   \\
oregon1\_010519       & 11.1k        & 22.7k    & 1.882     & 1.600   & 68.218   & 1.438  & 12.076                       & 14.199  & 0.333    & 15.800   \\
oregon2\_010421       & 11.1k        & 31.5k    & 2.917     & 2.002   & 68.057   & 1.899  & 10.813                       & 15.756  & 0.463    & 16.610   \\
oregon2\_010428       & 11.1k        & 31.4k    & 3.107     & 1.960   & 70.229   & 1.710  & 10.116                       & 16.035  & 0.448    & 18.380   \\
oregon2\_010505       & 11.2k        & 30.9k    & 2.703     & 2.122   & 70.168   & 1.550  & 11.447                       & 14.583  & 0.441    & 19.967   \\
oregon1\_010526       & 11.2k        & 23.4k    & 1.945     & 1.554   & 70.848   & 1.445  & 12.034                       & 15.067  & 0.330    & 16.206   \\
oregon2\_010512       & 11.3k        & 31.3k    & 3.060     & 1.585   & 70.707   & 1.687  & 10.229                       & 19.753  & 0.443    & 18.551   \\
oregon2\_010519       & 11.4k        & 32.3k    & 3.372     & 2.085   & 74.135   & 1.696  & 9.575                        & 15.482  & 0.436    & 19.041   \\
oregon2\_010526       & 11.5k        & 32.7k    & 3.253     & 2.011   & 77.051   & 1.639  & 10.061                       & 16.274  & 0.425    & 19.976   \\
ca-AstroPh            & 18.8k        & 198.1k   & 14.461    & 10.928  & 51.303   & 2.055  & 13.695                       & 18.123  & 3.860    & 96.365   \\
p2p-Gnutella25        & 22.7k        & 54.7k    & 0.548     & 0.468   & 0.340    & 0.171  & 99.790                       & 116.791 & 160.755  & 320.662  \\
ca-CondMat            & 23.1k        & 93.4k    & 3.090     & 1.996   & 9.496    & 0.990  & 30.239                       & 46.804  & 9.840    & 94.431   \\
as-caida20071105      & 26.5k        & 53.4k    & 6.659     & 4.417   & 139.697  & 2.238  & 8.016                        & 12.085  & 0.382    & 23.847   \\
p2p-Gnutella24        & 26.5k        & 65.4k    & 0.483     & 0.507   & 0.410    & 0.186  & 135.452                      & 129.009 & 159.475  & 352.204  \\
cit-HepTh             & 27.8k        & 352.3k   & 19.929    & 12.755  & 131.030  & 5.291  & 17.677                       & 27.619  & 2.689    & 66.586   \\
cit-HepPh             & 34.5k        & 420.9k   & 20.176    & 12.628  & 42.338   & 2.693  & 20.860                       & 33.328  & 9.941    & 156.291  \\
p2p-Gnutella30        & 36.7k        & 88.3k    & 0.593     & 0.507   & 0.381    & 0.198  & 148.951                      & 174.183 & 231.832  & 446.326  \\
email-Enron           & 36.7k        & 183.8k   & 16.768    & 7.101   & 180.731  & 4.599  & 10.963                       & 25.887  & 1.017    & 39.975   \\
loc-brightkite\_edges & 58.2k        & 214.1k   & 28.003    & 10.038  & 94.141   & 2.903  & 7.645                        & 21.326  & 2.274    & 73.749   \\
p2p-Gnutella31        & 62.6k        & 147.9k   & 1.116     & 0.930   & 0.431    & 0.203  & 132.508                      & 159.058 & 343.376  & 727.099  \\
soc-Epinions1         & 75.9k        & 405.7k   & 67.730    & 24.453  & 582.784  & 5.599  & 5.991                        & 16.593  & 0.696    & 72.472   \\
soc-Slashdot0811      & 77.4k        & 469.2k   & 42.498    & 14.202  & 146.617  & 3.968  & 11.040                       & 33.037  & 3.200    & 118.232  \\
soc-Slashdot0902      & 82.2k        & 504.2k   & 45.469    & 14.729  & 164.038  & 5.865  & 11.090                       & 34.233  & 3.074    & 85.977   \\
loc-gowalla\_edges    & 196.6k       & 950.3k   & 150.897   & 103.023 & 5332.719 & 14.762 & 6.298                        & 9.224   & 0.178    & 64.376   \\
amazon0302            & 262.1k       & 899.8k   & 11.741    & 7.625   & 10.346   & 1.275  & 76.634                       & 118.009 & 86.967   & 705.830  \\
email-EuAll           & 265.0k       & 364.5k   & 12.535    & 9.439   & 93.244   & 4.771  & 29.078                       & 38.616  & 3.909    & 76.389   \\
amazon0312            & 400.7k       & 2349.9k  & 56.524    & 33.074  & 131.514  & 5.975  & 41.573                       & 71.049  & 17.868   & 393.303  \\
amazon0601            & 403.4k       & 2443.4k  & 67.959    & 36.734  & 383.056  & 6.454  & 35.954                       & 66.516  & 6.379    & 378.594  \\
amazon0505            & 410.2k       & 2439.4k  & 60.062    & 34.748  & 140.891  & 6.161  & 40.615                       & 70.204  & 17.314   & 395.923  \\
roadNet-PA            & 1088.1k      & 1541.9k  & 2.894     & 2.821   & 0.627    & 0.644  & 532.736                      & 546.617 & 2458.775 & 2395.740 \\
roadNet-TX            & 1379.9k      & 1921.7k  & 3.955     & 3.696   & 0.812    & 0.837  & 485.881                      & 519.887 & 2367.159 & 2296.164 \\
roadNet-CA            & 1965.2k      & 2766.6k  & 5.733     & 4.956   & 1.149    & 1.189  & 482.601                      & 558.234 & 2407.210 & 2326.053 \\
cit-Patents           & 3774.8k      & 16518.9k & 195.765   & 138.447 & 82.991   & 35.532 & 84.382                       & 119.316 & 199.046  & 464.903  \\
\hline
\end{tabular}
}
\label{tab:48T_K3}
\end{table*}


==> Ktruss GraphChallenge 2019 cam ready plus IEEE copyright/prior_work.tex <==
Prior work in running K-truss has spanned CPU, GPU, shared memory, and distributed
memory systems. In addition, formulations of the algorithm have taken `think like a 
vertex,' linear algebraic, and other lenses.
Work by (NVIDIA et al.) in 2017 and 2018 in particular has looked at load-balancing 
K-truss through sorting vertices based on their degree (NEED TO VERIFY AND CITE!) \cite{}.
This approach could be used in complement with our proposed fine-grained parallel approach
for the eager K-truss algorithm.
(Mention Vignesh's work as well for sorting? What about graph partitioning?)

==> Ktruss GraphChallenge 2019 cam ready plus IEEE copyright/results.tex <==

% This section presents performance results of running the fine- and coarse-grained parallel
% versions of K-truss on both CPU and GPU using the same code base built on the Kokkos framework.
%Additionally, we select the value of K=3 because it encourages a %large number of iterations of the algorithm. 
%This is because the low K threshold allows many edges to survive %each pruning step, 
%causing K-truss to execute more iterations before reaching a steady state on the graph.

Table~\ref{tab:48T_K3} reports runtimes and ME/s results comparing between the coarse- and fine-grained using 48 CPU threads and on the GPU for the $K=3$ case. Due to space constraints, we do not also include a similar table for $K= K_{max}$. Where named in a plot, graphs are ordered from least number of edges (non-zero entries) to greatest, left to right. Where a plot bar for coarse-grained performance is not visible, vertical text is placed to state the ME/s rate achieved.

\subsection*{CPU Performance}

% ######################################
Fig. \ref{fig:thread_scaling} shows speedup of fine-grained versus coarse-grained parallelism for $K= K_{max}$. We omit the plot for $K=3$ except to state that speedups are slightly higher.

Speedup is above unity for most graphs, indicating that fine-grained has better performance per graph and per number of threads.
Some larger graphs show drops in speedup below unity for threads greater than 8.
This may be because $K=K_{max}$ aggressively prunes edges from the graph and reduces overall opportunities for parallelism.
Some graphs show peaks in speedup for 32 threads even if the 16 thread run has worse speedup than 8.
In future work we will examine the graphs' properties to determine causes for these peaks and troughs.
%
%For the $K=3$ case, however, the speedup for 32 threads often drops below that of 16 threads. 
%There are a few graphs that see increasing speedup as number of threads is increased: as20000102, loc-brightkite, oregon\_010512, p2p-Gnutella09, soc-Slashdot0811 and soc-Slashdot0902.
%
%For $K=K_{max}$, more of the speedups, especially at higher thread counts, see a decrease.
%The drops in speedup my be because this test case aggressively deletes more of the edges in the graph and may perform more iterations, and therefore more opportunity for parallelism in the fine-grained case is removed.
%Nonetheless, some graphs in that case actually have significantly higher speedup for the 32 thread case. WHY IS THIS????
%
%This indicates that for 8, 16, and 32 threads, the fine-grained implementation offers better or equal parallel scalability compared to the coarse-grained implementation. 
%A few graphs do show below one speedup at 16 or 32 threads (e.g. ca-HepTh, p2p-Gnutella\{04, 06, 24\}, roadNet-TX) suggesting that there are additional issues 
% ######################################


%These results suggest that the different approach to parallelism is indeed reducing load imbalance between parallel workers, thereby improving performance.


% \begin{figure}[ht]
% \centering
% \begin{subfigure}{\linewidth}
%     \includegraphics{plots/MEps with K=3.png}
%     \label{fig:K3_thread_scaling}
% \end{subfigure}
% \begin{subfigure}{\linewidth}
%     \includegraphics{plots/MEps with K=kmax.png}
%     \label{fig:Kmax_thread_scaling}
% \end{subfigure}
%     \caption{Comparison of coarse- and fine-grained parallel Kokkos implementations for K=3 (top) and K=K-max (bottom). The y-axis is measured in Millions of Edges processed per second, where the number of edges in the undirected graph is equal to the number of non-zero entries in the sparse matrix.}
%     \label{fig:thread_scaling}
% \end{figure}

% For $K=3$, the scaling of both implementations is sub-linear with respect to the number of threads. For $K=K_{max}$, however, both approaches suffer from a loss in performance at the highest number of threads (48). This is counter-intuitive because all threading cases represent use of physical cores and therefore do not involve hyper-threading. %Hence, there should be no increased contention in private caches or for processor compute resources. Instead of coming from core contention, 
% This performance drop may be due to lesser parallelism available in subsequent rounds of the K-truss algorithm as a higher $K$ value would mean many more edges are removed in earlier rounds.

%pruning the graph and the fine-grained method's reliance on the number of remaining non-zero elements in the graph. Since a higher K-max removes edges in larger numbers per iteration, the number of useful tasks that can still be computed in subsequent rounds decreases, causing a drop in available parallelism.
Fig. \ref{fig:CPU48T_all_graphs} shows performance of the CPU parallel implementations across all input graphs for 48 threads. 
Overall, the geometric mean speedup across graphs of the fine-grained parallel implementation over coarse-grained is 1.48x for $K=3$ and 1.26x for $K= K_{max}$, both for 48 threads.

% If space, maybe I need to discuss these results more (esp for larger graphs)

% TODO: fix plot titles, probably make span page width, possible remove one of the K cases.

\begin{figure*}
    \centering
    \includegraphics[height=1.75in,width=\textwidth]{plots/CPU_k=3_all_graphs.pdf}
    \includegraphics[height=2.5in,width=\textwidth]{plots/CPU_k=kmax_all_graphs.pdf}
    \caption{Performance for 48 CPU threads of coarse- and fine-grained implementations. Top: $K=3$. Bottom: $K=K_{max}$.}
    \label{fig:CPU48T_all_graphs}
\end{figure*}
\begin{figure*}
    \centering
    \includegraphics[height=1.75in,width=\textwidth]{plots/GPU_k=3_all_graphs.pdf}
    \includegraphics[height=2.5in,width=\textwidth]{plots/GPU_k=kmax_all_graphs.pdf}
    \caption{Performance on GPU of coarse- and fine-grained implementations. Top: $K=3$. Bottom: $K=K_{max}$.}
    \label{fig:GPU_all_graphs}
    \vspace{-2mm}
\end{figure*}

%\begin{figure}[ht]
%    \centering
%    \includegraphics[width=\linewidth]{plots/CPU_k=kmax_all_graphs.png}
%    \caption{Performance for 48 CPU threads of coarse- and fine-grained parallel implementations across all graphs. Performance is measured in Millions of Edges per Second and K is set to K-max for all graphs.}
%    \label{fig:CPU48T_all_graphs_K=kmax}
%\end{figure}

\subsection*{GPU Performance}
The difference in performance between the two parallelism approaches is much larger on the GPU.
Fig. \ref{fig:GPU_all_graphs} shows that, for the majority of the input graphs, the fine-grained implementation achieves significantly higher performance. For the case of $K=3$, the mean geometric speedup between the two parallel schemes on the GPU is 16.93x; for $K=K_{max}$, it is 9.97x.

%In fact, the coarse-grain implementation is often slower than either the CPU version.
%, while the fine-grained parallel GPU implementation typically performs better than either CPU version, with a mean geometric speedup of 1.92x over the fine-grained parallel CPU version. 
In addition to reducing load imbalance, executing in parallel over fine-grained tasks appears to benefit the GPU by increasing the amount of parallel work. This seems to be the case for the \textit{oregon} networks and \textit{as-caida20071105}, which have on the order 10,000 - 1,000 vertices and are among the smallest. 
However, larger graphs such as the \textit{roadNet} graphs and \textit{cit-Patents} show lower performance on the GPU. 
Determining the sources of these performance degradations will be the subject of future work. 
Overall, the fine-grained GPU implementation are 1.92x and 1.56x faster, for $K=3$ and $K_{max}$ respectively, than the fine-grained CPU implementation.

\input{plots/table.tex}

% TODO: fix plot titles, probably make span page width, possible remove one of the K cases.


%\begin{figure}[ht]
%    \centering
%    \includegraphics[width=\linewidth]{plots/GPU_k=kmax_all_graphs.png}
%    \caption{Performance on GPU of coarse- and fine-grained parallel implementations across all graphs. Performance is measured in Millions of Edges per Second and K is set to K-max for all graphs.}
%    \label{fig:GPU_all_graphs_K=kmax}
%\end{figure}

==> Ktruss GraphChallenge 2019 cam ready plus IEEE copyright/setup.tex <==
\subsection{Experimental Setup}
Input graphs from the Stanford Network Analysis Project (SNAP) \cite{snapnets} were downloaded from the GraphChallenge collection~\cite{graphchallenge:Isomorphism:2017}.
These graphs were made upper-triangular before being used as inputs.
Our CPU test platform was a single-node, dual-socket machine with 
two 24-core, 48-thread Intel Xeon Platinum 8160 CPUs, each operating at
2.10 GHz with a total of 187 GB of main memory.
Our GPU is an Nvidia Tesla V100 hosted on a second machine with a Power9 IBM processor. 
%Results are reported in Millions of Edges Per Second, and 
%The algorithm implementations 
%presented in the following section were run for each graph in our input 
%set for 10 trials, of which the mean performance metric is presented.
%All CPU thread scaling experiments were run on the Intel machine, while
%the GPU experiments were run on the Power9 / Tesla V100 platform.
%For thread scaling of the CPU implementations, values of 8, 16, 24, 32, 40, 
%and 48 threads were chosen in order to explore full use of the physical 
%cores on the Intel platform across both sockets.
% Use of hyperthreads was not explored...
Experiments were run for the cases when $K=3$, and $K=K_{max}$, i.e. the largest value of $K$ that returns a non-empty K-truss. 
The $K=3$ case is consistent with experiments in Bisson et al~\cite{Bisson2017, Bisson2018}.
Performance numbers are provided in terms of millions of edges processed per second 
(ME/s), and the mean of 10 trials is reported.
Correctness of all implementations was verified against the
reference K-truss code provided by Low et al.~\cite{low2018linear}.


%This metric is computed for a given graph as the number of edges in the original 
%graph divided by the amount of time spent computing the K-truss (for given $K$) of that graph. 


==> kokkos.tex <==
Performance portability, particularly for parallel algorithms,
is a major challenge for developers in HPC.
In this study, we seek to test our parallel-algorithmic approach to 
load balancing on both CPU and GPU platforms.
To code portability, we used the Kokkos parallelism framework to express 
flattened and nested parallel loops for kernels in eager K-truss. \cite{}
The Kokkos framework and runtime ?? enable such parallel applications to be written 
once and recompiled for shared-memory HPC platforms that used CPUs and GPUs.
Management of memory, including arbitration of atomic accesses and data layout 
are also handled by the Kokkos framework.

While in our testing we found that some performance was lost between our original
OpenMP C implementation of eager K-truss and the direct C++ port in Kokkos, 
the benefit was being able to test and deploy our implementations across both 
CPU and GPU hardware with minimal changes to code. 
Other frameworks for portable parallelism and performance include OpenCL, OpenACC,
and OpenMP itself \cite{}. 
We acknowledge these frameworks; however our objectives in this work do not include
a performance comparison between these different frameworks.


==> prior_work.tex <==
Prior work in running K-truss has spanned CPU, GPU, shared memory, and distributed
memory systems. In addition, formulations of the algorithm have taken `think like a 
vertex,' linear algebraic, and other lenses.
Work by (NVIDIA et al.) in 2017 and 2018 in particular has looked at load-balancing 
K-truss through sorting vertices based on their degree (NEED TO VERIFY AND CITE!) \cite{}.
This approach could be used in complement with our proposed fine-grained parallel approach
for the eager K-truss algorithm.
(Mention Vignesh's work as well for sorting? What about graph partitioning?)
